Convergence of AdaGrad for Non-convex Objectives: Simple Proofs and Relaxed Assumptions

We provide a simple convergence proof for AdaGrad optimizing non-convex objectives under only affine noise variance and bounded smoothness assumptions. The proof is essentially based on a novel auxiliary function $\xi$ that helps eliminate the complexity of handling the correlation between the numerator and denominator of AdaGrad's update. Leveraging simple proofs, we are able to obtain tighter results than existing results \citep{faw2022power} and extend the analysis to several new and important cases. Specifically, for the over-parameterized regime, we show that AdaGrad needs only $\mathcal{O}(\frac{1}{\varepsilon^2})$ iterations to ensure the gradient norm smaller than $\varepsilon$, which matches the rate of SGD and significantly tighter than existing rates $\mathcal{O}(\frac{1}{\varepsilon^4})$ for AdaGrad. We then discard the bounded smoothness assumption and consider a realistic assumption on smoothness called $(L_0,L_1)$-smooth condition, which allows local smoothness to grow with the gradient norm. Again based on the auxiliary function $\xi$, we prove that AdaGrad succeeds in converging under $(L_0,L_1)$-smooth condition as long as the learning rate is lower than a threshold. Interestingly, we further show that the requirement on learning rate under the $(L_0,L_1)$-smooth condition is necessary via proof by contradiction, in contrast with the case of uniform smoothness conditions where convergence is guaranteed regardless of learning rate choices. Together, our analyses broaden the understanding of AdaGrad and demonstrate the power of the new auxiliary function in the investigations of AdaGrad.

==> Tex_files/Intro_bak.tex <==
\section{Introduction}
\label{sec: intro}
Adaptive optimizers have been a great success in deep learning. Compared to stochastic gradient descent (SGD), adaptive optimizers use the gradient information of iterations to dynamically adjust the learning rate, which is observed to converge much faster than SGD in a wide range of deep learning tasks. Such a superiority has attracted numerous researchers to analyze the behavior of adaptive optimizers.

Among multitudinous adaptive optimizers, AdaGrad \citep{duchi2011adaptive} is considered to be the origin of the analysis. This is not only because AdaGrad is among the earliest optimizers and motivates most of the dominate optimizers nowadays, but also due to that the design of AdaGrad is quite simple: it simply accumulates the gradients of the past iterations and divide it to the current gradient to get the update. The psedo-codes of the norm version of AdaGrad (i.e., AdaGrad-Norm) and  AdaGrad are respectively presented in Algorithm \ref{alg: adagrad_norm} and Algorithm \ref{alg: adagrad}, where $g_t$ is required that $\mathbb{E}[g_t|\sigma (g_1,\cdots,g_{t-1})]=\nabla F(\bw_t)$ (latter we denote $\mathcal{F}_t \triangleq \sigma (g_1,\cdots,g_{t-1})$ ).

\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{AdaGrad-Norm}\label{alg: adagrad_norm}
    \hspace*{0.02in} {\bf Input:}
Objective function $f(\bw)$, learning rate $\eta>0$, initial point $\bw_{1} \in \mathbb{R}^d$, initial conditioner $\bnu_{1}\in \mathbb{R}^{+}$~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
    \begin{algorithmic}[1]
       \State \textbf{For} $t=1\rightarrow \infty$:
\State ~~~~~Generate stochastic gradient $g_t$
\State ~~~~~Calculate $\bnu_{t}=\bnu_{t-1}+\Vert g_t\Vert^2$
\State ~~~~~Update $\bw_{t+1}= \bw_{t}-\eta \frac{1}{\sqrt{\bnu_{t}}}  g_{t} $
\State \textbf{EndFor}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{AdaGrad}\label{alg: adagrad}
    \hspace*{0.02in} {\bf Input:}
Objective function $f(\bw)$, learning rate $\eta>0$, initial point $\bw_{1} \in \mathbb{R}^d$, initial conditioner $\bnu_{1}\in \mathbb{R}^{d,+}$~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
    \begin{algorithmic}[1]
       \State \textbf{For} $t=1\rightarrow \infty$:
\State ~~~~~Generate stochastic gradient $g_t$
\State ~~~~~Calculate $\bnu_{t}=\bnu_{t-1}+ g_t^{\odot 2}$
\State ~~~~~Update $\bw_{t+1}= \bw_{t}-\eta \frac{1}{\sqrt{\bnu_{t}}} \odot g_{t} $
\State \textbf{EndFor}
    \end{algorithmic}
\end{algorithm}
\end{minipage}


Despite the popularity of the adaptive optimizers and the simplicity of AdaGrad, the theoretical analysis of AdaGrad has not been well established. Specifically, over the non-convex objective functions, most of the existing analyses \cite{xxx} assume that the stochastic gradient $g_t$ is uniformly bounded across the iterations. Such an assumption does not hold even for quadratic functions, let alone deep neural networks. Moreover, the analysis of SGD does not require such an assumption.

The only exception is \citep{faw2022power}, which prove that AdaGrad-Norm converges assuming affine noise variance (c.f. our Assumption \ref{assum: affine}) and uniformly bounded smoothness (c.f. our Assumption \ref{assum: smooth}). These assumptions matches those of the state-of-art results of SGD. However, the results in \citet{faw2022power} still suffer from two drawbacks listed as follows. First, Assumption \ref{assum: affine} with $D_0=0$ is called the strong growth condition by existing literature \citep{xxx}, under which the averaged squared gradient $\frac{1}{T} \sum_{t=1}^T \Vert \nabla f(\bw_t) \Vert^2$ of SGD is shown to converge with rate $\mathcal{O}(\frac{1}{T})$, which is faster than the rate of SGD when $D_0\ne 0$. On the other hand, the rate of AdaGrad in \citep{faw2022power} is $\mathcal{O}(\frac{1}{\sqrt{T}})$ regardless of $D_0=0$ and there is a gap between the rates of AdaGrad and SGD. We believe that closing this gap is important, as the strong growth condition closely resembles the over-parameterized models, which is widely adopted in deep learning. Second, the proof in \citep{faw2022power} is rather complex (around 30 pages), which makes it hard to interpret the intuition behind and generalize it to the analysis of other optimizers.

We know that the convergence analysis of SGD under affine noise variance and $L$-smooth condition is quite simple. \textbf{What makes the analysis of AdaGrad so stiff?} It is due to the correlation between $g_t$ and $\bnu_t$. We illustrate this using AdaGrad-Norm. Specifically, with smoothness uniformly bounded by $L$ (i.e., Assumption \ref{assum: smooth}) the classical descent lemma yields
\begin{equation*}
 \mathbb{E}[f(\bw_{t+1})|\mathcal{F}_t]\le f(\bw_{t}) +\begin{matrix}\underbrace{  \mathbb{E}\left[\left\langle \nabla f(\bw_t), \bw_{t+1}-\bw_t \right\rangle|\mathcal{F}_t\right]}
   \\
    \text{First Order}
   \end{matrix} + \begin{matrix}\underbrace{\frac{L}{2}\mathbb{E}\left[ \left\Vert   \bw_{t+1}-\bw_t \right\Vert^2|\mathcal{F}_t\right]}
   \\
    \text{Second Order}
   \end{matrix}.
\end{equation*}
The $\bw_{t+1}-\bw_t$ is $-\eta g_t$ in SGD, thus the "First Order" term of SGD has a clear form, i.e., $-\eta \Vert \nabla f(\bw_t)\Vert^2 $. This term is negative and contributes to the decrease of $f$. However, due to the correlation between  $g_t$ and $\bnu_t$, the "First-Order" term of AdaGrad-Norm does not admit a clear form and we do not know whether it is negative or not. A common practice is to use a surrogate $\tilde{\bnu}_t$ of $\bnu_t$, which does not contain the information of $g_t$ and the correlation can be disentangled. Concretely,
\begin{align*}
   & \mathbb{E}\left[\left\langle \nabla f(\bw_t), \bw_{t+1}-\bw_t \right\rangle|\mathcal{F}_t\right]=\mathbb{E}\left[\left\langle \nabla f(\bw_t), -\eta \frac{g_t}{\sqrt{\bnu_t}} \right\rangle|\mathcal{F}_t\right]
    \\
    =&\mathbb{E}\left[\left\langle \nabla f(\bw_t), -\eta \frac{g_t}{\sqrt{\tilde{\bnu}_t}} \right\rangle|\mathcal{F}_t\right]
    + \mathbb{E}\left[\left\langle \nabla f(\bw_t), \eta g_t (\frac{1}{\sqrt{\tilde{\bnu}_t}}-\frac{1}{\sqrt{\bnu_t}}) \right\rangle|\mathcal{F}_t\right].
\end{align*}
The first term equals $-\eta \frac{\Vert \nabla f(\bw_t)\Vert^2}{\sqrt{\tilde{\bnu}_t}}$, which is negative and desired. However, the last term is an additional error term, which is very challenging to deal with. Existing results either assume bounded stochastic gradient to tackle it \citep{xxx}, or resolve it through complicated analysis \citep{faw2022power}.

In this paper, we propose a novel potential function which handles the error term easily. Specifically, our contributions can be summarized as follows:
\begin{itemize}
    \item We propose a novel potential function $\xi(t)=\frac{\Vert \nabla f(\bw_t) \Vert^2}{\sqrt{\bnu_t}}$ for the convergence analysis of AdaGrad(-Norm). This allows us to derive a much simpler proof (Theorem \ref{thm: adagrad_norm}) than the state-of-art result \citep{faw2022power} . Moreover, our conclusion is stronger: under strong growth condition, our convergence rate for AdaGrad-Norm is $\mathcal{O}(\frac{1}{T})$, which matches that of SGD and demonstrates that AdaGrad-Norm converges faster in the over-parameterized regime than in the non-over-parameterized regime.

    \item We then extend the analysis to AdaGrad by a coordinate version of $\xi(t)$  and show that the same conclusion holds as AdaGrad-Norm (Theorem \ref{alg: adagrad}), except that AdaGrad requires a coordinate-wise affine noise variance assumption (Assumption \ref{assum: coordinate_affine}). To the best of our knowledge, this is the first convergence result of AdaGrad without the requirement of bounded gradient norm.

    \item As the coordinate-wise affine noise assumption is stronger than the affine noise variance assumption, we seek to prove the convergence of AdaGrad under affine noise variance assumption. We consider randomly-reshuffled AdaGrad (RR AdaGrad), which is the version of AdaGrad used in deep learning practice, and show that RR AdaGrad does converge under affine noise variance assumption.

    \item We then step beyond the uniformly-bounded objective functions and consider a simple yet realistic non-uniformly-smooth condition called $(L_0,L_1)$-smooth condition (Assumption \ref{assum: non-smooth}), which allows the local gradient Lipschitz coefficient to grow with the gradient norm. We prove that AdaGrad(-Norm) still converges under $(L_0,L_1)$-smooth condition, but requires the learning rate to be smaller than a threshold. We also provide a counterexample over which AdaGrad with a large learning rate diverges.  Together, our results demonstrate that AdaGrad can overcome the non-uniform smoothness, but lose the tuning-free ability in this case.
\end{itemize}

The rest of this paper is organized as follows. In Section \ref{sec: preliminary}, we define notations and provide assumptions; in Section \ref{sec: motivation}, we demonstrate the motivation to use the potential function; in Section \ref{sec: adagrad_norm}, we derive the convergence result of AdaGrad-Norm under $L$-smooth condition; in Section \ref{sec: adagrad}, we extend the result to AdaGrad; in Section \ref{sec: non-uniform}, we analyze the convergence of AdaGrad(-Norm) under $(L_0,L_1)$-smooth condition.
